OPENGRASP-LITE Version 1.0: A Tactile Artificial Hand with a Compliant Linkage Mechanism

Recent research has seen notable progress in the development of linkage-based artificial hands. While previous designs have focused on adaptive grasping, dexterity and biomimetic artificial skin, only a few systems have proposed a lightweight, accessible solution integrating tactile sensing with a compliant linkage-based mechanism. This paper introduces OPENGRASP LITE, an open-source, highly integrated, tactile, and lightweight artificial hand. Leveraging compliant linkage systems and MEMS barometer-based tactile sensing, it offers versatile grasping capabilities with six degrees of actuation. By providing tactile sensors and enabling soft grasping, it serves as an accessible platform for further research in tactile artificial hands.

==> Images/main_control_state_machine.tex <==

\begin{tikzpicture}[shorten >=1pt,node distance=\manControlFSMScale*3cm,on grid,auto,bend angle=10, scale=\manControlFSMScale, every node/.style={scale=\manControlFSMScale}]
    \tikzstyle{stateNormal}=[style=state, minimum width=1cm];
    
    \node[stateNormal,initial by diamond] (s0) {$s_0$};
    \node[stateNormal] (s1) at ($(s0) + (0,-2.13)$) {$s_1$};
    \node[stateNormal] (s2) [right=of s1] {$s_2$};
    \node[stateNormal] (s3) [above right=of s2] {$s_3$};
    \node[stateNormal] (s4) [below=of s3] {$s_4$};
    \node[stateNormal] (s5) [below left=of s2] {$s_5$};
    
    \path[->] (s0) edge node{a/1} (s1);
    \path[->] (s1) edge [loop below] node {b/2} ();
    \path[->] (s1) edge node [above] {c/0} (s2);
    \path[->] (s2) edge [bend left] node [rotate=45,above] {d/3} (s3);
    \path[->] (s3) edge [bend left] node [rotate=45,below] {d/0} (s2);
    \path[->] (s3) edge node [rotate=90,below] {f/4} (s4);
    \path[->] (s4) edge node [rotate=-22.5,below] {f,d/0} (s2);

    
    \path[->] (s2) edge [bend left] node [rotate=45,below] {d/5} (s5);
    \path[->] (s5) edge [bend left] node [rotate=45,above] {d,f/0} (s2);

    
    \path[->] (s3) edge [loop left] node {e/3} ();
    \path[->] (s4) edge [loop below] node {e/4} ();
    \path[->] (s5) edge [loop right] node {e/5} ();
    %\draw(7.0,0.25)rectangle(15.75,-2.75);
    \draw (-1,-5) node (states) {}
    ++ (0, 0.0) node[anchor=west] {\textbf{States}}
    ++ (0,-0.5) node[anchor=west] {$s_0$: Init}
    ++ (0,-0.5) node[anchor=west] {$s_1$: Calibrate}
    ++ (0,-0.5) node[anchor=west] {$s_2$: Stop}
    ++ (0,-0.5) node[anchor=west] {$s_3$: Prepare}
    ++ (0,-0.5) node[anchor=west] {$s_4$: Close}
    ++ (0,-0.5) node[anchor=west] {$s_5$: Open};
    
    \draw (states) ++ (2.5,0) node (inputs) {}
    ++ (0, 0.0) node[anchor=west] {\textbf{Inputs}}
    ++ (0,-0.5) node[anchor=west] {$a$: Init}
    ++ (0,-0.5) node[anchor=west] {$b$: Calib Prepared}
    ++ (0,-0.5) node[anchor=west] {$c$: Calib Finished}
    ++ (0,-0.5) node[anchor=west] {$d$: Grasp Update}
    ++ (0,-0.5) node[anchor=west] {$e$: Speed Update}
    ++ (0,-0.5) node[anchor=west] {$f$: All Stopped};
    
    \draw (inputs) ++ (3.25,0) node (outputs) {}
    ++ (0, 0.0) node[anchor=west] {\textbf{Outputs}}
    ++ (0,-0.5) node[anchor=west] {$0$: Stop}
    ++ (0,-0.5) node[anchor=west] {$1$: Prepare Calib}
    ++ (0,-0.5) node[anchor=west] {$2$: Calibrate}
    ++ (0,-0.5) node[anchor=west] {$3$: Position $\omega_\text{Prep}$}
    ++ (0,-0.5) node[anchor=west] {$4$: Position $\omega_\text{Close}$}
    ++ (0,-0.5) node[anchor=west] {$5$: Position $\omega_\text{Open}$};

    \draw($(states) + (-0.2,-0.25)$)--++(8.8,0);
    \draw($(inputs) + (0,0.25)$) --++ (0,-3.5);
    \draw($(outputs) + (0,0.25)$) --++ (0,-3.5);

\end{tikzpicture}

==> Tables/Finger_dimensions.tex <==
\begin{table}[h]
\centering
\caption{Finger Phalange Dimensions (mm) }
\vspace{-0.5\baselineskip}
\begin{tabular}{||c|c|c|c||}
 \hline
 Proximal & Middle & Distal & Total Length\\ [0.5ex] 
 \hline\hline
 36.0 & 23.5 & 21.0 & 80.5 \\
 \hline
\end{tabular}
\label{tab: finger_dimensions}
\end{table}
